Hardware-Software Contracts for Secure Speculation

Since the discovery of Spectre, a large number of hardware mechanisms for secure speculation has been proposed. Intuitively, more defensive mechanisms are less efficient but can securely execute a larger class of programs, while more permissive mechanisms may offer more performance but require more defensive programming. Unfortunately, there are no hardware-software contracts that would turn this intuition into a basis for principled co-design. In this paper, we put forward a framework for specifying such contracts, and we demonstrate its expressiveness and flexibility. On the hardware side, we use the framework to provide the first formalization and comparison of the security guarantees provided by a representative class of mechanisms for secure speculation. On the software side, we use the framework to characterize program properties that guarantee secure co-design in two scenarios traditionally investigated in isolation: (1) ensuring that a benign program does not leak information while computing on confidential data, and (2) ensuring that a potentially malicious program cannot read outside of its designated sandbox. Finally, we show how the properties corresponding to both scenarios can be checked based on existing tools for software verification, and we use them to validate our findings on executable code.

==> overview-figure.tex <==
\begin{figure*}[ht!]
        \centering
               \begin{tikzpicture}
                \node (table) {  
                   { \begin{tabular}{l l  l }
                     \multirow{2}{*}{\textbf{Software}}    & \multirow{2}{*}{Program $p$} & \emph{Proof obligation (goal 1):} $p$ satisfies \emph{constant-time}  with respect to $\interfSem{\cdot}$ \\
                     &    &  \emph{Proof obligation (goal 2):} $p$ satisfies \emph{sandboxing}  with respect to $\interfSem{\cdot}$\\
                     \multicolumn{3}{c}{\textbf{Contract}  $\interfSem{\cdot}$}\\
                     \multirow{2}{*}{\textbf{Hardware}}    & \multirow{2}{*}{Platform $\CtxMuarchSem{\cdot}{}$} &  \multirow{2}{*}{\emph{Proof obligation:}    $\CtxMuarchSem{\cdot}{}$ satisfies  $\interfSem{\cdot}$ }\\
                     & & \\ %
                    \end{tabular}
                   }
                };
                \draw[black!50,dashed,rounded corners]
  ($(table.north west)$)
  rectangle 
  ($(table.south east) !.6! (table.north east)$);
  \draw [black!50,dashed,rounded corners]
  ($(table.south west) !.4! (table.north west)$)
  rectangle 
  ($(table.south east)$);
            \end{tikzpicture}

    \caption{Overview of our approach. The contract $\interfSem{\cdot}$ provides an interface between hardware (here, platform $\CtxMuarchSem{\cdot}{}$) and software (here, program $p$) and it splits responsibilities for preventing side-channels between hardware and software.
    On the hardware side, a designer needs to prove that its platform $\interfSem{\cdot}{}$ complies with a contract $\CtxMuarchSem{\cdot}{}$. On the software side, a contract $\interfSem{\cdot}$ induces proof obligations for programs $p$ to be secure on any platform $\CtxMuarchSem{\cdot}{}$ satisfying $\interfSem{\cdot}$.
    }\label{figure:overview}
\end{figure*}



